Logic Blog 2021

The blog has several entries on group theory interacting with computability and wider logic, several open questions, and an entry on undecidability in physics.

==> sections2021/On_BD_theorem_Yu.tex <==
\section{Yu: On  Besicovitch sets}
   \begin{theorem}[Besicovitch]
 There is a null set $A\subseteq \mathbb{R}^2$  contains   a unit segment in each orientation.
  \end{theorem}
  \begin{proof}
 Let $  A=\{(x,a+bx)\in [0,1]^2\mid b\in [0,1]\wedge a\in L_{\omega_1^b}[b]  \}$.
 
 Clearly $A$ contains   a unit segment in each orientation.
 
  \end{proof}
  
  The shortage of the current proof is that it is even more complicated (or not simpler) than the original proof.

